2-Level Quasi-Planarity or How Caterpillars Climb (SPQR-)Trees

Given a bipartite graph $G=(V_b,V_r,E)$, the $2$-Level Quasi-Planarity problem asks for the existence of a drawing of $G$ in the plane such that the vertices in $V_b$ and in $V_r$ lie along two parallel lines $\ell_b$ and $\ell_r$, respectively, each edge in $E$ is drawn in the unbounded strip of the plane delimited by $\ell_b$ and $\ell_r$, and no three edges in $E$ pairwise cross. We prove that the $2$-Level Quasi-Planarity problem is NP-complete. This answers an open question of Dujmovi\'c, P\'{o}r, and Wood. Furthermore, we show that the problem becomes linear-time solvable if the ordering of the vertices in $V_b$ along $\ell_b$ is prescribed. Our contributions provide the first results on the computational complexity of recognizing quasi-planar graphs, which is a long-standing open question. Our linear-time algorithm exploits several ingredients, including a combinatorial characterization of the positive instances of the problem in terms of the existence of a planar embedding with a caterpillar-like structure, and an SPQR-tree-based algorithm for testing the existence of such a planar embedding. Our algorithm builds upon a classification of the types of embeddings with respect to the structure of the portion of the caterpillar they contain and performs a computation of the realizable embedding types based on a succinct description of their features by means of constant-size gadgets.

==> packages.tex <==
%\usepackage{fullpage}

\usepackage{epsfig}
\usepackage{gensymb}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{subfigure}
%\usepackage{times}
\usepackage{hyperref}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{paralist}
\usepackage{amsmath,amscd,amssymb,german}
%\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage[scaled]{helvet}
\usepackage{dsfont}
\usepackage[T1]{fontenc}
\usepackage[ansinew]{inputenc}
\usepackage{paralist}
\usepackage{wrapfig}


%%%%%%%%%ABBREVIATIONS%%%%%%%%%%
\newcommand{\twopcp}{$2$-PCP\xspace}
\newcommand{\bTWObesc}{{\sc b2pbesc}\xspace}
\renewcommand{\dots}{...}

%%%%%%%%%COMPLEXITY%%%%%%%%%%
\newcommand{\NP}{$\mathcal{NP}$\xspace}
\newcommand{\PP}{$\mathcal{P}$\xspace}
\renewcommand{\NP}{$\mathcal{NP}$}
\newcommand{\NPH}{\mbox{\NP-hard}\xspace}
\newcommand{\NPC}{\mbox{\NP-complete}\xspace}
\newcommand{\npc}{\mbox{\NP-complete}}
\newcommand{\NPCN}{\mbox{\NP-completeness}\xspace}
\newcommand{\npcn}{\mbox{\NP-completeness}}
\newcommand{\NPHN}{\mbox{\NP-hardness}\xspace}
\newcommand{\nphn}{\mbox{\NP-hardness}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{blue}{rgb}{0.274,0.392,0.666}
\definecolor{red}{rgb}{1,0.3,0.3}
\definecolor{green}{rgb}{0,0.588,0.509}

\newcommand{\red}[1]{{{#1\xspace}}}
\newcommand{\blue}[1]{{{#1\xspace}}}
\newcommand{\green}[1]{{{#1\xspace}}}

\newcommand{\bbep}{{\sc Bipartite Book-Embedding}\xspace}
\newcommand{\bbe}{{\sc BBE}\xspace}
\newcommand{\lp}{{\sc Level Planarity}\xspace}
\newcommand{\bookinstance}[1]{$G^{#1}({V_1^{#1}} \cup {V_2^{#1}}, E^{#1})$\xspace}
\newcommand{\Vr}[1]{${V_1^{#1}}$\xspace}
\newcommand{\Vb}[1]{${V_2^{#1}}$\xspace}

\newcommand{\clpshort}{{\sc CL-Planarity}\xspace}


\newcommand{\Gint}{$G_{\cap}$\xspace}
\newcommand{\Gr}[1]{$\red{G^{#1}_1}$\xspace}
\newcommand{\Gb}[1]{$\blue{G^{#1}_2}$\xspace}
\newcommand{\clinstance}[1]{$(V^{#1},E^{#1},\gamma^{#1})$\xspace}
\newcommand{\clp}{{\sc Cyclic Level Planarity}\xspace}
\newcommand{\tlp}{{\sc {\em $T$}-Level Planarity}\xspace}

\newcommand{\tlinstance}[1]{$(V^{#1},E^{#1},\gamma^{#1},\mathcal{T}^{#1})$\xspace}
\newcommand{\stinstance}[1]{$\langle G^{#1},\sigma^{#1} \rangle$\xspace}
\newcommand{\betp}{{\sc Betweenness}\xspace}


\newcommand{\sefeinstance}[1]{$\langle\red{G^{#1}_1},\blue{G^{#1}_2}\rangle$\xspace}
\newcommand{\sefe}{{\sc sefe}\xspace}
\newcommand{\tuba}{$^\dag$} \newcommand{\rome}{$^{\diamond}$} \newcommand{\kit}{$^{\circ}$}

\newcommand{\cpllong}{Clustered Planarity with Linear Saturators\xspace}
\newcommand{\cpl}{{\sc cpls}\xspace}

\newtheorem{observation}{Observation}
\newcommand{\image}[1]{\includegraphics[scale=0.3]{#1}}
\newcommand{\plot}[1]{\includegraphics[scale=0.55]{#1}}
\newcommand{\remove}[1]{}
\newcommand{\rephrase}[3]{\noindent\textbf{#1 #2}.~\emph{#3}}

\newcommand{\ignaz}[1]{\marginpar{{\color{red}Ignaz says: }#1}}

\newenvironment{proofsketch}
{\noindent{\em Proof sketch:}}{\hspace*{\fill}\qed\par\vspace{2mm}}

\iffalse
\renewenvironment{proof}
{{\bf Proof:}}{\hspace*{\fill}$\Box$\par\vspace{2mm}}
\newenvironment{proofx}
{{\bf Proof of Theorem~\ref{th:sefe-main}:}}{\hspace*{\fill}$\Box$\par\vspace{2mm}}
\newenvironment{proofy}
{{\bf Proof of Lemma~\ref{le:splittingpoints}:}}{\hspace*{\fill}$\Box$\par\vspace{2mm}}
\fi

\let\doendproof\endproof
\renewcommand{\endproof}{\qed\doendproof}
